Quantum state tracking and control of a single molecular ion in a thermal environment

Understanding molecular state evolution is central to many disciplines, including molecular dynamics, precision measurement, and molecule-based quantum technology. Details of the evolution are obscured when observing a statistical ensemble of molecules. Here, we reported real-time observations of thermal radiation-driven transitions between individual states ("jumps") of a single molecule. We reversed these "jumps" through microwave-driven transitions, resulting in a twentyfold improvement in the time the molecule dwells in a chosen state. The measured transition rates showed anisotropy in the thermal environment, pointing to the possibility of using single molecules as in-situ probes for the strengths of ambient fields. Our approaches for state detection and manipulation could apply to a wide range of species, facilitating their uses in fields including quantum science, molecular physics, and ion-neutral chemistry.

==> scratch.tex <==
\noindent{\textbf{\large Supplementary text}}

\bigskip

\noindent{\underline{Molecular state detection, projection, and pumping using quantum-logic spectroscopy}}

In a quantum-logic spectroscopy (QLS) operation, information about the internal state of a spectroscopy ion ($^{40}$CaH$^+$) is coherently transferred onto a logic ion ($^{40}$Ca$^+$) via their shared harmonic normal modes of motion within the ion trap potential. 
First, Ca$^+$ is prepared in the state $| D\rangle \equiv | D_{5/2}, m_a = -5/2 \rangle$ and the axial out-of-phase motional mode in its ground state ($|n = 0 \rangle$). Here, $m_a$ is the magnetic quantum number of Ca$^+$, and $n$ is the harmonic oscillator quantum number for the motion. Then, a sideband transition that attempts to change the internal state of CaH$^+$ while adding a quantum of excitation to the motion ($ |\mathcal J \rangle | 0 \rangle \rightarrow |\mathcal J' \rangle | 1 \rangle $) is driven by a pair of far-detuned 1064 nm laser beams in a Raman configuration. The two beams have $\sigma^-$ and $\pi$ polarizations, respectively, which drives transitions between $|\mathcal J \rangle = |J, m, \xi \rangle $ and $|\mathcal J' \rangle = | J, m\pm1, \xi'\rangle $. Next, a motion-subtracting sideband transition is attempted on Ca$^+$ ($ | D \rangle | 1 \rangle \rightarrow | S \rangle | 0 \rangle $). Here, $| S \rangle \equiv | S_{1/2}, m_a = -1/2 \rangle$ is a bright state under the excitation of a 397 nm laser while repumped by a 866 nm laser, and can be distinguished from the dark state $| D \rangle$ with high fidelity. The detection of atomic fluorescence at the end of the sequence indicates that the molecular transition was successfully driven, which implies detection of the molecule in $|\mathcal J \rangle$. This also non-destructively heralds the molecule's projection into $|\mathcal J' \rangle$. Each projection attempt takes a total of 5.8 ms, which consists of ground-state cooling of the axial out-of-phase mode (4.1 ms), sideband operations on the atomic and molecular ions (1.5 ms), and fluoresence detection on the atomic ion (0.2 ms).

\begin{figure} [t!]
\centering
\includegraphics[width=1.0\textwidth]{J1&2_pumping_sequences.pdf}
    \caption{\small``pump \& project" pulse sequences for detecting in $J = 1$ (a) and $J = 2$ (b) manifolds. Red and black arrows represent pumping and projection transitions, respectively. The circled numbers indicate the order in which the transitions are driven. For $J = 2$, we use ``carrier'' transitions (purple arrows), which change only the internal state the molecule but not the motion, to transfer the probabilities from states which suffer from low pumping efficiency to states which can be efficiently pumped. The energy level structures are to scale and calculated for $^{40}$CaH$^+$ in the presence of co-aligned DC magnetic ($B = 6.5 $ G) and RF electric ($E_{\text{RF}} = 1300 $ V/m) fields. A scale bar marking 10 kHz is provided in both (a) and (b).}
\label{J1_2PumpingSequences}
\end{figure}

While QLS in principle allows the detection/projection of the molecule in any state, most Raman transitions in $^{40}$CaH$^+$ are too weak and/or not spectrally resolved from other transitions to allow unambiguous identification of the detected/projected state. The exceptions include transitions between $|J, m = -J - 1/2, - \rangle$ and $|J, m = -J + 1/2, - \rangle$, which are strong and distinctive in frequency from one another and all other Raman transitions \cite{chou2017preparation}, and are referred to as ``signature" transitions. Given these characteristics, we detect the molecular state by first combining the probability of finding the molecule in each sublevel of a given $J$-manifold, $P_{\mathcal{J}}$, into $|J, m = -J - 1/2, - \rangle$ via QLS-based pumping \cite{chou2017preparation}, and then attempt a projection using the signature transition. 
In each pumping step, we drive a $\pi$-pulse on a motion-adding sideband transition $|\mathcal J \rangle = |J, m, \xi \rangle |n = 0\rangle \rightarrow |\mathcal J' \rangle = | J, m\pm1, \xi'\rangle |n = 1\rangle$, and then perform ground-state cooling on the motion ($|n = 1\rangle \rightarrow |n = 0\rangle$).
This introduces dissipation in the system that combines the probabilities in $|\mathcal J \rangle$ into $|\mathcal J' \rangle$. 
This detection method is referred to as ``pump \& project", and the pulse sequences are illustrated schematically in Figure \ref{J1_2PumpingSequences} for $J = 1$ and 2. Their durations are 20.4 and 32.3 ms, respectively. Following the full pumping sequence, the probability in $|J, m = -J - 1/2, - \rangle$ is $\zeta \sum_{\mathcal{J}\in J} P_{\mathcal{J}}$, where $\zeta$ is the overall pumping efficiency. For the illustrated pulse sequences, we measure $\zeta = 0.95(5)$ for $J = 1$ and $0.90(5)$ for $J = 2$. When a pumping sequence similar to that for $J = 2$ is applied to $J \geq 3$, we currently find $\zeta < 0.5$, thus preventing the efficient detection of these manifolds.

\bigskip
\noindent{\underline{State-resolved detection of the $J = 1$ manifold}}

In this section, we describe the procedure used to detect individual states of the $J = 1$ manifold and observe quantum jumps from $J = 0$ to 1 (Figure 2B).
After preparing the molecule in either sublevel of $J = 0$ and the logic ion and the motion in $|D\rangle |0 \rangle$, we detect each sublevel of $J = 1$ (\textit{e.g.}, $| 1, -3/2, -\rangle$) by projecting it towards a neighboring sublevel (\textit{e.g.}, $| 1, -1/2, -\rangle$). Upon a successful initial projection (\textit{e.g.}, $| 1, -3/2, -\rangle \rightarrow | 1, -1/2, -\rangle$), two additional projections (\textit{e.g.}, $| 1, -1/2, -\rangle \rightarrow | 1, -3/2, -\rangle$ and $| 1, -3/2, -\rangle \rightarrow | 1, -1/2, -\rangle$) are required to confirm the result of the first projection. We observed that the multiple projections suppress the false positive probability to $< 0.2~\%$. Primary sources for false positive events in our system include heating of the axial out-of-phase mode ($|D\rangle |0 \rangle \rightarrow |D\rangle | 1 \rangle$) and spontaneous decay of Ca$^{+}$ ($|D\rangle | 0 \rangle \rightarrow |S\rangle | 0 \rangle$), both of which will result in Ca$^{+}$ in the $|S \rangle$ state after the motion-subtracting atomic sideband and a false positive signal. Without loss of generality, we detect the sublevels in the order $| 1, -3/2, -\rangle$, $| 1, -1/2, +\rangle$, $| 1, -1/2, -\rangle$, $| 1, +1/2, +\rangle$, $| 1, +1/2, -\rangle$, and $| 1, +3/2, +\rangle$.

\begin{figure}[t!]
\centering
\includegraphics[width=0.75\textwidth]{figure_J1_sublevel_readout_efficiency.pdf}
    \caption{\small Probability of detecting the molecule in each of the 6 sublevels of $J = 1$ following an initial preparation in one of the sublevels. The numbers in the parentheses represent 1SD uncertainty from the measurements.}
\label{J1ReadoutEfficiencies}
\end{figure}

Another source of imperfection during our detection is cross-talk, whereby the occupation of one sublevel is falsely assigned to another one. Contributing factors to cross-talk include the fact that some neighboring sublevels share the same pair of molecular sidebands for detection (\textit{e.g.}, $| 1, -3/2, -\rangle$ and $| 1, -1/2, -\rangle$, $| 1, -1/2, +\rangle$ and $| 1, +1/2, +\rangle$), non-ideal spectral separation between some of the sidebands (especially those within the ``$+$'' manifold), and the requirement for multiple consecutive detections which may shuffle the molecule to a different sublevel than the one it started in. To characterize the effect of cross-talks on the detection, we performed experiments where the molecular ion is deliberately prepared in a given sublevel of $J = 1$, and all 6 sublevels are detected using a sequence identical to that used to monitor quantum jumps from $J = 0$ to 1. The resulting state histograms are displayed in Figure \ref{J1ReadoutEfficiencies}, and are used to convert the raw data into that shown in Figure 2B. The ``$+$'' states suffer from worse cross-talk due to the smaller frequency separation between the detection sidebands compared to those used for the ``$-$'' states.

\bigskip
\noindent{\underline{Estimating rates/probabilities for transitions between $J = 0$ and 1}}

In this section, we discuss the calculation of the relative rates (or, equivalently, probabilities) of transitions from either sublevel of $J = 0$ to different sublevels of $J = 1$ by an isotropic, nuclear spin conserving process (\textit{e.g.}, background gas collision, blackbody radiation) (Figure 2B). Any sublevel of $^{40}$CaH$^+$ $| \mathcal{J} \rangle = |J, m, \xi \rangle$ may be written in the basis $| J, m_J \rangle | I, m_I \rangle$ as
\begin{equation}
    |\mathcal{J} \rangle = c^{-}_{\mathcal{J}} |J, m_J = m + 1/2\rangle | I = 1/2, m_I = -1/2 \rangle + c^{+}_{\mathcal{J}} |J, m_J = m - 1/2\rangle | I = 1/2, m_I = 1/2 \rangle,
\end{equation}
where $c^{-}$ and $c^{+}$ are the state amplitudes for the $ m_I = -1/2$ and $ m_I = 1/2$ components of the state, respectively, and $m_J \in \{ -J, -J + 1, ..., J - 1, J \}$. Consider a transition between two sublevels $\mathcal{J}$ and $\mathcal{J}'$. The transition matrix element can be expressed as $M_{\mathcal{J},\mathcal{J'}} = \langle \mathcal{J} | \mathbf{M} | \mathcal{J'} \rangle$, where $\mathbf{M}$ is the operator corresponding to the process, \textit{e.g.,} dipole operator for TR, potential energy operator for collisions. Assuming $\mathbf{M}$ acts only on the rotational but not the nuclear spin part of the state, we have
\begin{equation} \label{TME}
    M_{\mathcal{J},\mathcal{J'}} = c^{-}_{\mathcal{J}}c^{-}_{\mathcal{J'}} \langle J, m_J = m + 1/2 | \mathbf{M} | J', m_J' = m' + 1/2 \rangle + c^{+}_{\mathcal{J}}c^{+}_{\mathcal{J'}} \langle J, m_J = m - 1/2 | \mathbf{M} | J', m_J' = m' - 1/2 \rangle.
\end{equation}
Now consider transitions between $J = 0$ and 1. Since $c^{-}_{|0, -1/2, - \rangle} = c^{+}_{|0, 1/2, + \rangle} = 1$ and $c^{+}_{|0, -1/2, - \rangle} = c^{-}_{|0, 1/2, + \rangle} = 0$, we have $M_{|0, -1/2, - \rangle, |\mathcal{J'} \in J = 1 \rangle} = c^{-}_{|\mathcal{J'} \in J = 1\rangle} \langle 0, 0 | \mathbf{M} | 1, m_J' \rangle$, and $M_{|0, 1/2, + \rangle,|\mathcal{J'}\in J = 1\rangle} = c^{+}_{|\mathcal{J'}\in J = 1\rangle} \langle 0, 0 | \mathbf{M} | 1, m_J'\rangle$. Without \textit{a priori} knowledge about the details of the process, we assume, for the purpose of this estimate, that it is isotropic. This means that $\langle 0, 0 | \mathbf{M} | 1, m_J'\rangle$ has the same value for $m_j' = -1, 0,$ and 1, and the strength of the process (\textit{e.g.}, number of background gas molecules colliding with CaH$^+$, energy density of the TR field) is equal for the transitions from $m_j = 0$ to $m_j' = -1, 0,$ and 1. In this case, $M_{|0, \pm1/2, \pm \rangle,|\mathcal{J'}\in J = 1\rangle} \propto c^{\pm}_{|\mathcal{J'}\in J = 1\rangle}$, and the corresponding transition rates are $ \Gamma_{|0, \pm1/2, \pm \rangle,|\mathcal{J'}\in J = 1\rangle} \propto |M_{|0, \pm1/2, \pm \rangle,|\mathcal{J'}\in J = 1\rangle}|^2 \propto |c^{\pm}_{|\mathcal{J'}\in J = 1\rangle}|^2$. The rates are in turn proportional to the probabilities of finding the molecule in $| \mathcal{J'} \in J = 1 \rangle$ following its initialization in one of the two $| \mathcal{J} \in J = 0 \rangle $ sublevels, and we calculate these probabilities according to $P_{|0, \pm1/2, \pm \rangle,|\mathcal{J'}\in J = 1\rangle} = | c^{\pm}_{|\mathcal{J'}\in J = 1\rangle} |^2 /\sum_{|\mathcal{J'}\in J = 1\rangle} | c^{\pm}_{|\mathcal{J'}\in J = 1\rangle} |^2 $. Their values are displayed in Tab. \ref{tab:CGSJ0to1} along with the values of $c^{\pm}_{|\mathcal{J'}\in J = 1\rangle}$ from which they derive. The $c^{\pm}_{|\mathcal{J'}\in J = 1\rangle}$ are calculated by diagonalizing the Hamiltonian for CaH$^+$ under an intentionally applied external DC magnetic field of 6.5 G, and a co-aligned residual RF electric field of 1300 V/m in amplitude which cannot be compensated \cite{collopy2023effects}.

\begin{table}
\centering
\addtolength{\leftskip} {-2cm}
\addtolength{\rightskip}{-2cm}
\begin{threeparttable}
\caption{\small \label{tab:CGSJ0to1} State amplitudes for $J = 1$ sublevels ($c^{\pm}_{\mathcal{J'}\in J = 1}$) and the corresponding probabilities of undergoing a transition from $| 0, \pm1/2 \rangle$ to $J = 1$ sublevels ($P_{|0, \pm1/2, \pm \rangle,|\mathcal{J'}\in J = 1\rangle}$) for an isotropic, nuclear spin conserving process.}
\small
\begin{tabular}{lcccccc}
\hline\hline
 & $| 1, -3/2, - \rangle$ & $| 1, -1/2, - \rangle$ & $| 1, 1/2, - \rangle$ & $| 1, -1/2, + \rangle$ & $| 1, 1/2, + \rangle$ & $| 1, 3/2, + \rangle$ \\
\hline
$c^{-}_{|\mathcal{J'}\in J = 1\rangle}$ & 1 & 0.9846 & 0.9894 & 0.1749 & 0.1450 & 0 \\
$P_{|0, -1/2, - \rangle,\mathcal{J'}\in J = 1}$ & 0.3333 & 0.3231 & 0.3263 & 0.0102 & 0.0070 & 0 \\
$c^{+}_{|\mathcal{J'}\in J = 1\rangle}$ & 0& $-0.1749$ & $-0.1450$ & 0.9846& 0.9894& 1 \\
$P_{|0, 1/2, + \rangle,\mathcal{J'}\in J = 1}$ & 0  &  0.0102  &  0.0070  &  0.3231  &  0.3263  &  0.3333 \\
\hline\hline
\end{tabular}
\end{threeparttable}
\end{table}

\bigskip

\noindent{\underline{Rates for transitions driven by thermal radiation}}

The TR-driven transition rate between two individual sublevels $| \mathcal{J} \rangle = | J, m, \xi \rangle$ and $| \mathcal{J'} \rangle = | J', m', \xi' \rangle$ is given by 
\begin{equation} \label{Gamma_TR}
    \Gamma_{\mathcal{J} \rightarrow \mathcal{J'}} = \rho^\textrm{TR}_{\mathcal{J},\mathcal{J'}} B_{\mathcal{J},\mathcal{J'}} + A_{\mathcal{J},\mathcal{J'}},    
\end{equation}
where $\rho_\textrm{TR}$ is energy density for the component of TR driving the $| \mathcal{J} \rangle \rightarrow |\mathcal{J'} \rangle$ transition, $B_{\mathcal{J},\mathcal{J'}} = \frac{2 \pi^2}{3 h^2 \epsilon_0} |\mu_{\mathcal{J},\mathcal{J'}}|^2 $ is the Einstein coefficient for stimulated absorption or emission, and $A_{\mathcal{J},\mathcal{J'}} = \frac{16 \pi^3 \nu^3}{3 h \epsilon_0 c^3} |\mu_{\mathcal{J},\mathcal{J'}}|^2 $ is the Einstein coefficient for spontaneous emission, which is only nonzero for $J' < J$. $\mu_{\mathcal{J},\mathcal{J'}}$ is given by Eq. \ref{TME}, in which the generic operator $\mathbf{M}$ is replaced by the dipole operator $\vec{\mu}$. We can evaluate $\mu_{\mathcal{J},\mathcal{J'}}$ using state amplitudes obtained from solving the molecular Hamiltonian, the previously measured ground state permanent dipole moment of $^{40}$CaH$^+$ $\mu_{\textrm{CaH}^+}$ = 5.34(19) Debye \cite{collopy2023effects}, as well as $\langle J, m_J | \vec{\mu} | J', m_J' \rangle$ calculated using formulas for the matrix elements of pure rotational transitions (Ref. \cite{townes2013microwave} p. 22). According to dipole selection rules, $\langle J, m_J | \vec{\mu} | J', m_J' \rangle \neq 0$ for $J' = J \pm 1$ and $m_J' = m_J, m_J\pm 1$.

Using Eq. \ref{Gamma_TR}, we can estimate the rates for TR-driven transitions given a specific model for $\rho_\textrm{TR}$, \textit{e.g.,} Planck's law for blackbody radiation $\rho_{\textrm{BBR}}(\nu, T) = \frac{8\pi h \nu^3}{c^3} \frac{1}{\exp{[h\nu/(k_B T)]} - 1}$. To obtain comparisons for the measured rates $\Gamma^{\textrm{meas.}}_{J = 0 \rightarrow 1}$ and $\Gamma^{\textrm{meas.}}_{J = 1 \rightarrow 2}$ (Figure 4A, upper panel), we calculate $\Gamma^{\textrm{BBR}}_{J = 0 \rightarrow 1}$ and $\Gamma^{\textrm{BBR}}_{J = 1 \rightarrow 2}$ by setting $\rho_{\textrm{TR}} = \rho_{\textrm{BBR}}$ and summing over the transition rates from the relevant sublevels (Figure 4A, lower panel).
For either $| \mathcal{J} \in J = 0 \rangle $, we find $\Gamma^{\textrm{BBR}}_{J = 0 \rightarrow 1} = \rho_\textrm{BBR}(\nu = 285~\textrm{GHz}, T) \frac{2 \pi^2}{3 h^2 \epsilon_0} \sum_{\mathcal{J'}\in J = 1} |\mu_{\mathcal{J}, \mathcal{J'} }|^2 $, where $ \sum_{\mathcal{J'}\in J = 1} |\mu_{\mathcal{J}, \mathcal{J'} }|^2 = \mu^2_{\textrm{CaH}^+} $. Similarly, for any $| \mathcal{J} \in J = 1 \rangle $, we find $\Gamma^{\textrm{BBR}}_{J = 1 \rightarrow 2} = \rho_\textrm{BBR}(\nu = 570~\textrm{GHz}, T) \frac{2 \pi^2}{3 h^2 \epsilon_0} \sum_{\mathcal{J'}\in J = 2} |\mu_{\mathcal{J}, \mathcal{J'} }|^2 $, where $ \sum_{\mathcal{J'}\in J = 2} |\mu_{\mathcal{J}, \mathcal{J'} }|^2 = \frac{2}{3} \mu^2_{\textrm{CaH}^+} $. The uncertainty in the measured $\mu_{\textrm{CaH}^+}$ propagates into the calculated values for $\Gamma^{\textrm{BBR}}_{J = 0 \rightarrow 1}$ and $\Gamma^{\textrm{BBR}}_{J = 1 \rightarrow 2}$. 
By comparing $\Gamma^{\textrm{meas.}}$ and $\Gamma^{\textrm{BBR}}$ along with their associated uncertainties, we find the range of values for $T$ over which the blackbody model agrees with our measurements (Figure 4A, upper panel).

\begin{table}
\centering
\addtolength{\leftskip} {-2cm}
\addtolength{\rightskip}{-2cm}
\begin{threeparttable}
\caption{\small \label{tab:energyDensityRatio} Transition probability and rate data used to calculate the ratio between $\sigma^-$- and $\pi$-polarized TR presented in Figure 4B. All error bars represent 1 SD uncertainty.}
\small
\begin{tabular}{cccccc}
\hline\hline
 Data type & $\sigma^-$ transition & value & $\pi$ transition & value & $\rho^\textrm{TR}_{\sigma^-}/{\rho^\textrm{TR}_{\pi}}$ \\
\hline
Probability & $|0, -1/2, -\rangle \rightarrow |1, -3/2, -\rangle$ & 0.342(17) & $|0, -1/2, -\rangle \rightarrow |1, -1/2, -\rangle$ & 0.259(17) & 1.28(10) \\
Probability & $|0, 1/2, +\rangle \rightarrow |1, -1/2, +\rangle$ & 0.358(17) & $|0, 1/2, +\rangle \rightarrow |1, 1/2, +\rangle$ & 0.299(23) & 1.21(11) \\
Rate        & $|1, -3/2, -\rangle \rightarrow |0, -1/2, -\rangle$ & 0.0799(77) s$^{-1}$ & $|0, -1/2, -\rangle \rightarrow |0, -1/2, -\rangle$ & 0.0472(66) s$^{-1}$ & 1.68(30) \\
      &  & 0.0828(81) s$^{-1}$ &   & 0.0579(61) s$^{-1}$ & 1.41(21) \\
      &   & 0.0802(36) s$^{-1}$ &   & 0.0507(36) s$^{-1}$ & 1.57(14) \\
\hline\hline
\end{tabular}
\end{threeparttable}
\end{table}


We may also use Eq. \ref{Gamma_TR} to derive the energy density of TR from measured transition rates or probabilities.
We do so to obtain the ratios between the energy densities of $\sigma^-$- and $\pi$-polarized components of TR at $\sim$ 285 GHz, ${\rho^\textrm{TR}_{\sigma^-}}/{\rho^\textrm{TR}_{\pi}}$, which are presented in Figure 4B. For $J = 0 \rightarrow 1$ transitions, the term $A_{\mathcal{J},\mathcal{J'}}$ is zero, and we have
\begin{equation*}
    \frac{\rho^\textrm{TR}_{\mathcal{J} \in J = 0,\mathcal{J'} \in J = 1}}{\rho^\textrm{TR}_{\mathcal{J} \in J = 0,\mathcal{J''} \in J = 1}} = \frac{\Gamma^{\textrm{meas.}}_{\mathcal{J} \in J = 0,\mathcal{J'} \in J = 1}}{\Gamma^{\textrm{meas.}}_{\mathcal{J} \in J = 0,\mathcal{J''} \in J = 1}} \frac{|\mu_{\mathcal{J} \in J = 0,\mathcal{J''} \in J = 1}|^2}{|\mu_{\mathcal{J} \in J = 0,\mathcal{J'} \in J = 1}|^2}.
\end{equation*}
 Using the transition probabilities presented in Figure 2B (which are proportional to rates) and the state amplitudes from Tab. \ref{tab:CGSJ0to1}, we calculate the energy density ratios for the cases $\{|\mathcal{J}\rangle = |0, -1/2,-\rangle\}, |\mathcal{J'}\rangle = |1, -3/2, -\rangle, |\mathcal{J''\rangle} = |1, -1/2, -\rangle\}$ and $\{|\mathcal{J}\rangle = |0, 1/2,+\rangle, |\mathcal{J'}\rangle = |1, -1/2, +\rangle, |\mathcal{J''}\rangle = |1, 1/2, +\rangle\}$, which correspond to the purple and green arrow pairs in the inset of Figure 4B, respectively. For $J = 1 \rightarrow 0$ transitions, we use  Eq. \ref{Gamma_TR} to convert the measured rates for the transitions $|1,-3/2,-\rangle\rightarrow|0,-1/2,-\rangle$ and $|1,-1/2,-\rangle\rightarrow|0,-1/2,-\rangle$ (blue arrows in Figure 4B inset) into corresponding energy densities for $\sigma^-$- and $\pi$-polarized TR, and then take their ratio.
The rates for these transitions are obtained from the molecular state control experiments summarized in Figure 3. The molecule is prepared in either $|1,-3/2,-\rangle$ or $|1,-1/2,-\rangle$, the number of transitions to $|0,-1/2,-\rangle$ is recorded over the duration of the sequence, and the rate is calculated by dividing the number of transitions by the time the molecule spent in the prepared $J = 1$ sublevel.
The rate data are collected over three sets on different days, yielding the three blue square data points in Figure 4B. All data used to calculate the energy density ratios are presented in Tab. \ref{tab:energyDensityRatio}.

Molecules possess a variety of different transitions and can be used to sense different parts of the thermal radiation frequency spectrum, and even different polarization components. Similar to atom-based sensors, molecules have the potential for high-precision sensing with the core element of each sensor identically constructed by nature. Such a sensor can be in-situ probes for the thermal environment for precision measurements based on neutral and charged atoms, such as optical atomic clocks.

To accurately measure the properties of thermal radiation with this scheme, the sampling rate for the molecular state needs to be much higher than the transition rates so the jumps between molecular states are all detected. Other mechanisms that can cause such jumps will also need to be characterized to constrain their effects on the measurement. These pose limitations on the dynamic range.

\bigskip
\noindent{\underline{TR-driven transitions to vibrationally excited states}}

While we are primarily concerned with TR-driven transitions between rotational manifolds within the ground vibrational state ($v = 0$) in our state tracking experiments, there exists finite rates of transitions to vibrationally excited states ($v'$). In this section, we estimate these rates from first principles. Specifically, we are interested in the rates of TR-driven transitions from the target manifold of our tracking protocol $\{v = 0, J = 1\}$ to all allowed excited rovibrational manifolds, which are limited by the dipole selection rule to $\{v', J' = 0\}$ and $\{v', J' = 2\}$. For the purpose of this estimate, we work under the assumption that the thermal environment is described by an ideal blackbody at 300 K.

To facilitate the discussions of rovibrational transitions, we label each state as $| v, J, m, \xi \rangle$, where $v$ is the vibrational quantum number. Due to dipole selection rules of TR-driven transitions, $| v = 0, J = 1, m, \xi \rangle$ can only couple to $| v', J', m', \xi'\rangle$ for which $J' - J = \pm 1$ and $m' - m = 0, \pm 1$.
The transition dipole moment (TDM) of a rovibrational transition is given by the expression \cite{simons1997quantum}
\begin{equation}
    \mu_{| v, J, m, \xi \rangle \rightarrow | v', J', m', \xi' \rangle } = \langle v, J, m, \xi | \vec{\mu} | v', J', m', \xi' \rangle = \langle v | \mu | v' \rangle \langle J, m_J, \xi | \hat{\mu} | J', m_J', \xi' \rangle \\
\end{equation}
where $\vec{\mu}$ is the (electronically averaged) dipole moment operator, $\mu$ is its magnitude along the direction of the Ca-H bond, and $\hat{\mu}$ is a unit vector specifying the orientation of the bond (\textit{i.e.}, $\vec{\mu} = \mu\cdot \hat{\mu}$). $\mu_{v,v'} = \langle v | \mu | v' \rangle$ is the vibrational dipole matrix element, whose diagonal elements represent the permanent dipole moment (PDM) of CaH$^+$ in various vibrational states, and off diagonal elements represent the TDMs between vibrational states. $\hat{\mu}_{\{J, m_J, \xi\},\{J', m_J', \xi'\}} = \langle J, m_J, \xi | \hat{\mu} | J', m_J', \xi' \rangle$ is the rotational factor whose value is, to first order, independent of the vibrational state.

\begin{table}
\centering
\addtolength{\leftskip} {-2.5cm}
\addtolength{\rightskip}{-2cm}
\begin{threeparttable}
\caption{\small \label{tab:rovibTDM} Rates of rovibrational transitions and the parameters used to calculate them. $\mu_{v,v'}$ vibrational dipole matrix element (values are from \textit{ab initio} calculations performed by \blue{P. N. Plessow (private communication)}, which are within $\sim10\%$ of those from Ref. \cite{abe2010ab}); $\nu$: rovibrational transition frequency; $\rho$: TR energy density (BBR model at 300 K); $\Gamma$: transition rate.}
\small
\begin{tabular}{cccccccc}
\hline\hline
 $v'$ & $\mu_{v,v'}$ & $\nu_{\{0,1\}\rightarrow\{v',0\}}$ & $\rho(\nu_{\{0,1\}\rightarrow\{v',0\}}, 300~\text{K})$ & $\Gamma_{\{0,1\}\rightarrow\{v',0\}}$ & $\nu_{\{0,1\}\rightarrow\{v',2\}}$ & $\rho(\nu_{\{0,1\}\rightarrow\{v',2\}}, 300~\text{K})$ & $\Gamma_{\{0,1\}\rightarrow\{v',2\}}$ \\
 ~ & ($e \cdot a_0$) & (THz) & (J m$^{-3}$ Hz$^{-1}$) & (s$^{-1}$) & (THz) & (J m$^{-3}$ Hz$^{-1}$) & (s$^{-1}$) \\ 
\hline
 0 & 2.09 & 0.285 & $3.07\times10^{-22}$ & 0.0549 & 0.570 & $1.20\times10^{-21}$ & 0.429 \\
 1 & $6.70\times10^{-2}$  & 44.2 & $4.66\times10^{-20}$ & $8.48\times10^{-3}$ & 44.8 & $4.31\times10^{-20}$ & 0.0157 \\
 2 & $2.01\times10^{-2}$ & 87.1 & $3.76\times10^{-22}$ & $6.16\times10^{-6}$ & 87.7 & $3.38\times10^{-22}$ & $1.11\times10^{-5}$ \\
 3 & $4.02\times10^{-3}$ & 129 & $1.57\times10^{-24}$ & $1.02\times10^{-9}$ & 129 & $1.39\times10^{-24}$ & $1.82\times10^{-9}$ \\
 4 & $1.13\times10^{-3}$ & 169 & $5.64\times10^{-27}$ & $2.91\times10^{-13}$ & 170 & $5.00\times10^{-27}$ & $5.16\times10^{-13}$ \\
 5 & $3.62\times10^{-4}$ & 208 & $2.09\times10^{-29}$ & $1.11\times10^{-16}$ & 208 & $1.84\times10^{-29}$ & $1.95\times10^{-16}$ \\
\hline\hline
\end{tabular}
\end{threeparttable}
\end{table}

We use Eq. \ref{Gamma_TR} to calculate the rates of rovibrational transitions driven by TR, from a sublevel of $\{ v = 0, J = 1 \}$ to all sublevels of $\{ v', J' = 0, 2\}$ (the effects of rovibrational transitions from $\{ v = 0, J = 0 \}$ and $\{ v = 0, J = 2 \}$ can be ignored, since the molecule are only found in these manifolds during recoveries, and the recoveries account for $\lesssim 4\%$ of the total duration where the state is tracked). We suppress the quantum numbers $m$ and $\xi$ in state labeling, since the rate is identical for any sublevel of $\{ v = 0, J = 1 \}$.
The calculated rates, along with the dipole moments and TR energy densities used in the calculations, are presented in Tab. \ref{tab:rovibTDM}. At 300 K, non-negligible vibrational transitions occurs only to $v' = 1$. These transitions result in leakage in the probability to find the molecule in the tracked subspace and impacts the performance of our state tracking protocol, which we discuss in the following section.

\bigskip
\noindent{\underline{State tracking experiment timing}}

\begin{figure}[h!]
\centering
\includegraphics[width=1.00\textwidth]{state_tracking_timing.pdf}
    \caption{\small \textbf{Timing of the state tracking experiment}. Center panel: an example of experiment timing during a period of continuous state tracking beginning with projection of the state into $| 1, -1/2, - \rangle$ and ends with the failure to recovery the state back to $J = 1$. Upper panel: an individual time step which consists of a waiting period for coherent operations and two QLS detections from $| 1, -1/2, - \rangle$ and $| 1, -3/2, - \rangle$, respectively. Lower panel: the recovery sequence, in which the state is searched in four sub-manifolds: the ``$-$" states of $J = 1$, the ``$+$" states of $J = 1$, the ``$-$" states of $J = 2$, the ``$+$" states of $J = 2$, and finally the two sublevels of $J = 0$. }
\label{stateTrackingTiming}
\end{figure}

In this section we present the timing of various procedures during the state tracking and control experiment presented in Figure 3. A schematic timing diagram of the experimental sequence is presented in Figure \ref{stateTrackingTiming}. The center panel represents a period of continuous state tracking, which begins with projection of the state into $| \mathcal{J}_i \rangle = | 1, -1/2, - \rangle$ and ends with the failure to recovery the state back to $J = 1$. This corresponds to a green block from Figure 3D. The majority of the sequence consists of a repetition of individual time steps, the details of which are shown in the upper panel of Figure \ref{stateTrackingTiming}. Each individual time step consists of a waiting period of 25 ms (reserved for coherent operations on the molecular state in future experiments), and two QLS detections from $| 1, -1/2, - \rangle$ and $| 1, -3/2, - \rangle$, respectively. The repetition of the time steps is interrupted by a failure to detect in both of these sublevels, which triggers the execution of a sequence of pulses to attempt recovery of the state. The recovery sequence is shown in the lower panel of Figure \ref{stateTrackingTiming}. The sequence uses the ``pump \& project" method to search for the state in four sub-manifolds: the ``$-$" states of $J = 1$ (using pulses \textcircled{4}, \textcircled{5}, and \textcircled{6} in Figure \ref{J1_2PumpingSequences}(a)), the ``$+$" states of $J = 1$ (using pulses \textcircled{1} -- \textcircled{6} in Figure \ref{J1_2PumpingSequences}(a)), the ``$-$" states of $J = 2$ (using pulses \textcircled{1} -- \textcircled{4} and \textcircled{14} in Figure \ref{J1_2PumpingSequences}(b)), and the ``$+$" states of $J = 2$ (using pulses \textcircled{5} -- \textcircled{14} in Figure \ref{J1_2PumpingSequences}(b)). Positive detections in $J = 1$ will automatically resets the state to $| 1, -1/2, - \rangle$ by design of the pulse sequence, while positive detection in $J = 2$ will be followed by a $\sim$570 GHz microwave $\pi$-pulse to drive a $J = 2\rightarrow1$ transition. Additionally, the sequence detects the two sublevels of $J = 0$ by coherently transferring any probability in $|0, -1/2, - \rangle$ ($|0, 1/2, + \rangle$) to $| 1, -3/2, - \rangle$ ($| 1, -1/2, - \rangle$) via a $\sim$285 GHz microwave $\pi$-pulse and then attempting a projection. If the state is recovered at the end of any of the above stages, the recovery sequence terminates and the experiment resumes repetition of the individual time steps. We allow the execution of up to three complete recovery sequences before declaring failure to recover the state, at which point the system goes back to waiting for a projection in the subspace $J = \{0,1,2\}$.

\bigskip
\noindent{\underline{Limitations on state tracking performance}}

The performance of our state tracking and control protocol (Figure 3D) can be measured in terms of the the average duration by which we can continuously keep the molecule in $J = 1$  ($\overline{T}_{\text{track}}$). This duration is limited by processes which cause transitions (``leakage'') out of the tracked subspace $J \in \{0, 1, 2\}$. In this section, we discuss the leakage channels and estimate their rates. We work under the assumption of a 300 K blackbody thermal environment, which approximately describes our system. Given the molecular structure of CaH$^+$, we identify two leakage channels: rotational leakage and vibrational leakage (Figure \ref{stateTrackingLeakage}). We label each  rotational manifold in the ground vibrational state as $J$, and those in the excited vibrational states as $\{ v, J \}$, where $v$ is the vibrational quantum number. For both channels, we consider the leakage to be irreversible once the molecule reaches the $ J = 3 $ manifold. For rotational leakage, the dominant path is $J = 1 \xrightarrow{\text{TR}} J = 2 \xrightarrow{\text{TR}} J = 3$. For vibrational leakage, the dominant path is $J = 1 \xrightarrow{\text{TR}} \{ v = 1, J = 2 \} \xrightarrow[\text{decay}]{\text{Spont.}} J = 3$.

\begin{figure}[t!]
\centering
\includegraphics[width=1.00\textwidth]{state_tracking_leakage_v3.pdf}
    \caption{\small \textbf{Leakages from tracked subspace during state tracking}. (a) Rotational leakage: the molecule undergoes TR-driven transitions (red and blue solid arrows) via the path $J = 1 \xrightarrow{\text{TR}} J = 2 \xrightarrow{\text{TR}} J = 3$. This can occur either during an individual time step of the experiment (a second order process), or during the attempt to recover the state from $J = 2$ back to $J = 1$ (a first order process).
    (b) Vibrational leakage: undergoes TR-driven transitions (red solid arrows) from $J = 1$ to the vibrationally excited manifolds $\{v' = 1, J' = 0\}$ and $\{v' = 1, J' = 2\}$. From both manifolds, the molecule can decay (via spontaneous emission) back to $J = 1$ (green dotted arrows), which does not result in a leakage. From $\{v' = 1, J' = 2\}$, the molecule can also decay to $J = 3$ (blue dotted arrows), resulting in a leakage. The branching fraction for the leakage decay ($ \{ v = 1, J = 2 \} \xrightarrow[\text{decay}]{\text{Spont.}} J = 3$) is $9/19$. The rates ($\Gamma$) of the relevant TR-driven transitions are labeled next to the arrows indicating the transitions.
    }
\label{stateTrackingLeakage}
\end{figure}

To estimate the leakage rate due to these channels, we first consider the probabilities in various relevant manifolds coupled to $J = 1$ by TR after an individual time step ($\Delta t$) during the tracking experiment. Each time step consists of the wait time, $t_{\text{wait}}$, and the time to check whether the state is still in $J = 1$, $t_{J = 1, \text{check}}$. $t_{J = 1, \text{check}}$ consists primarily of the time to detect in the sublevels $| 1, -1/2, - \rangle$ and $| 1, -3/2, - \rangle$ (5.8 ms each), but also the time for the occasional recoveries from the $J = 1$ ``$-$" states and $J = 1$ ``$+$" states as part of the recovery sequence. The latter process adds, on average, $\sim 1$ ms to each time step (Figure \ref{stateTrackingTiming}, upper panel). The relevant manifolds are $J = 3$, as well as those that can additionally couple to $J = 3$, which include $J = 2$ and $\{ v = 1, J = 2 \}$. In the beginning of a time step, the molecule is initialized in $J = 1$. We can solve for the probabilities using the set of approximate rate equations
\begin{equation} \label{rateEqns1}
    \begin{split}
        \dot{P}_{J = 2}(t) &= \Gamma_{J = 1\rightarrow2} P_{J = 1}(t) \\
        \dot{P}_{J = 3}(t) &= \Gamma_{J = 2\rightarrow3} P_{J = 2}(t) \\
        \dot{P}_{\{v = 1, J = 2\}}(t) &= \Gamma_{\{0,1\} \rightarrow \{1,2\}} P_{J = 1}(t), \\
    \end{split}
\end{equation}
with the initial condition 
$\{P_{J = 1}(0) = 1,~P_{J = 2}(0) = 0,~P_{J = 3}(0) = 0,~P_{\{v = 1, J = 2\}}(0) = 0\}$.
Note that here we have ignored any back flow of probability to $J = 1$ based on the criteria that each time step is very short compared to the inverses of the relevant rates.
To the lowest order, the solutions to Eq. \ref{rateEqns1} at the end of each time step ($t = \Delta t$) are

\begin{equation} \label{rateEqns2}
    \begin{split}
        \Delta P_{J = 2} = P_{J = 2}(\Delta t) &= \Gamma_{J = 1\rightarrow2} \Delta t \\
        \Delta P_{J = 3} = P_{J = 3}(\Delta t) &= \frac{1}{2}\Gamma_{J = 1\rightarrow2}\Gamma_{J = 2\rightarrow3} \Delta t^2 \\
        \Delta P_{\{v = 1, J = 2\}} = P_{\{v = 1, J = 2\}}(\Delta t) &= \Gamma_{\{0,1\} \rightarrow \{1,2\}} \Delta t. \\
    \end{split}
\end{equation}

Now we consider the probability of additional loss from $J = 2$ and $\{ v = 1, J = 2 \}$ to $J = 3$. For $J = 2$, loss to $J = 3$ can occur due to TR-driven transition during the recovery, and the probability is, to first order, $\Gamma_{J = 1\rightarrow3} t_{J = 2,\text{rec.}}$. Here, $t_{J = 2,\text{rec.}}$ represents the average time the recovery sequence takes to bring the molecule back to $J = 1$. Note that $t_{J = 2,\text{rec.}}$ is not deterministic as more than one recovery attempt is occasionally required to reset the state back to $J = 1$. We therefore use the average value of $J = 2$ recovery times measured during the tracking experiments for our estimates. For $\{ v = 1, J = 2 \}$, there is a branching fraction of $R_{\{1, 2 \}\rightarrow J = 3}$ of spontaneous decays to $J = 3$, while the rest of the decays are back to $J = 1$. As such, the total loss probability from $J = 1$ to $J = 3$ after a time step is

\begin{equation}  \label{lossPerTimeStep}
    \begin{split}
        \Delta P_{\text{loss}} &= (\Gamma_{J = 2\rightarrow3} t_{J = 2,\text{rec.}}) \Delta P_{J = 2} + \Delta P_{J = 3} + R_{\{1, 2 \}\rightarrow J = 3} \Delta P_{\{v = 1, J = 2\}} \\
        &= \Gamma_{J = 1\rightarrow2} t_{J = 2,\text{rec.}} \Gamma_{J = 2\rightarrow3}\Delta t + \frac{1}{2}\Gamma_{J = 1\rightarrow2}\Gamma_{J = 2\rightarrow3} \Delta t^2 + R_{\{1, 2 \}\rightarrow J = 3} \Gamma_{\{0,1\} \rightarrow \{1,2\}} \Delta t
    \end{split}
\end{equation}

After each successful recovery the initial conditions of Eq. \ref{rateEqns1} are restored and the protocol proceeds with the next time step. The probability for the loss to occur in the $n$-th time steps is
\[
P_{\text{loss}}(n) = (1 - \Delta P_{\text{loss}})^{n - 1}\Delta P_{\text{loss}},
\]
and the average step at which the loss occurs is
\[
\langle n \rangle = \sum_{n = 1}^{\infty} n P_{\text{loss}}(n) = \frac{1}{\Delta P_{\text{loss}}}.
\]
Therefore the average time for continuous tracking is
\begin{equation}
    \begin{split}
        \overline{T}_{\text{track}} = \langle n \rangle \Delta t &= \frac{\Delta t}{\Gamma_{J = 1\rightarrow2} \Delta t~\Gamma_{J = 2\rightarrow3} t_{J = 2,\text{rec.}} + \frac{1}{2}\Gamma_{J = 1\rightarrow2}\Gamma_{J = 2\rightarrow3} \Delta t^2 + R_{\text{vib.}\rightarrow J = 3} \Gamma_{\text{vib.}} \Delta t} \\
        &= \left(\Gamma_{J = 1\rightarrow2} \Gamma_{J = 2\rightarrow3} t_{J = 2,\text{rec.}} + \frac{1}{2}\Gamma_{J = 1\rightarrow2}\Gamma_{J = 2\rightarrow3} \Delta t + R_{\text{vib.}\rightarrow J = 3} \Gamma_{\text{vib.}}\right)^{-1} \\
        &= \left[\Gamma_{J = 1\rightarrow2} \Gamma_{J = 2\rightarrow3} \left(t_{J = 2,\text{rec.}} + \frac{\Delta t}{2}\right) + R_{\{1, 2 \}\rightarrow J = 3} \Gamma_{\{0,1\} \rightarrow \{1,2\}}\right]^{-1},
    \end{split}
\end{equation}
and the effective rate of loss from $J = 1$ during tracking is
\begin{equation} \label{GammaLoss}
        \Gamma_{\text{loss}} = \overline{T}^{-1}_{\text{track}} = \Gamma_{J = 1\rightarrow2} \Gamma_{J = 1\rightarrow3} \left(t_{J = 2,\text{rec.}} + \frac{\Delta t}{2}\right) + R_{\{1, 2 \}\rightarrow J = 3} \Gamma_{\{0,1\} \rightarrow \{1,2\}} = \Gamma_{\text{loss}}^{\text{rot.}} + \Gamma_{\text{loss}}^{\text{vib.}}.
\end{equation}
Here, $\Gamma_{\text{loss}}^{\text{rot.}} = \Gamma_{J = 1\rightarrow2} \Gamma_{J = 1\rightarrow3} \left(t_{J = 2,\text{rec.}} + \Delta t/2\right)$ represents rotational leakage, and \\$\Gamma_{\text{loss}}^{\text{vib.}} = R_{\{1, 2 \}\rightarrow J = 3} \Gamma_{\{0,1\} \rightarrow \{1,2\}}$ represents vibrational leakage. For the tracking experiment shown in Figure 3, we estimate $\Gamma_{\text{loss}}^{\text{rot.}} = 0.0268$ s$^{-1}$,  $\Gamma_{\text{loss}}^{\text{vib.}} = 0.0074$ s$^{-1}$, and $\Gamma_{\text{loss}} = 0.0343$  s$^{-1}$, using the calculated rates ($\Gamma_{J = 1 \rightarrow 2} = 0.4290$ s$^{-1}$, $\Gamma_{J = 2 \rightarrow 3} = 0.8480$ s$^{-1}$, $\Gamma_{\{0,1\} \rightarrow \{1,2\}} = 0.0157$ s$^{-1}$), the calculated branching fraction ($R_{\{1, 2 \}\rightarrow J = 3} = 9/19 \approx 0.474$), and the known times from the tracking protocol ($t_{\text{wait}} = 25$ ms, $t_{J = 1, \text{check}} = 12.56$ ms, $\Delta t = t_{\text{wait}} + t_{J = 1, \text{check}} = 37.56$ ms, $t_{J = 2, \text{rec.}} = 55.04$ ms). The total loss rate corresponds to an average continuous tracking time of $\overline{T}_{\text{track}} = \Gamma^{-1}_{\text{loss}} = $ 29.1 s, comparable to the experimental value of 35.5 s. Eq. \ref{GammaLoss} shows that, to the lowest orders, $\Gamma_{\text{loss}}$ has a linear dependence on the wait time for coherent operations (Recall that $\Delta t = t_{\text{wait}} + t_{J = 1, \text{check}}$).

Finally, we note that both rotational and vibrational leakages populate the state $J = 3$. As such, further improvements in the state tracking duration can be achieved by incorporating the detection of $J = 3$ into our state recovery sequence. To this end, efficient method to pump the $J = 3$ manifold must be developed. After pumping, the probabilities in $J = 3$ can be transferred to $J = 1$ via a Raman transition, as we have demonstrated in Ref. \cite{chou2020frequency} using a pair of frequency combs.

\bigskip
\noindent{\underline{Applicability of the state tracking and control protocol to other molecular ion species}}

To apply the state tracking and control protocol demonstrated here to another molecular ion species, efficient access of molecular state information is essential. Currently this is realized by transferring state information via the coupled harmonic motion between the ions. The closer the coupled motion is to the quantum mechanical ground state the better signal-to-noise ratio in molecular state detection. This results in a limitation on the mass-to-charge ratio ($m/z$) of the molecular ion for a given atomic ion, since in systems of large $m/z$ mismatches certain motional modes are not amenable to cooling to the ground state. However, recent experiments have demonstrated the transfer of excitations in modes not amenable to ground state cooling to those which are in systems of atomic ions with large $m/z$ mismatches \cite{hou2024indirect}. This represents a promising approach to overcoming the $m/z$ limitations in single molecule QLS experiments. 

“Signature” transitions with distinctive frequencies also improve signal-to-noise ratio of the detections and enable state-specific operations as well as polarization selectivity. While such transitions exist within rotational manifolds, transitions between rotational manifolds and even vibrational manifolds for a molecular species of interest could be considered for this purpose. The transition strengths and lifetimes of the involved states will need to accommodate the coherent operations on the molecule.
